PoCo: Point Context Cluster for RGBD Indoor Place Recognition

We present a novel end-to-end algorithm (PoCo) for the indoor RGB-D place recognition task, aimed at identifying the most likely match for a given query frame within a reference database. The task presents inherent challenges attributed to the constrained field of view and limited range of perception sensors. We propose a new network architecture, which generalizes the recent Context of Clusters (CoCs) to extract global descriptors directly from the noisy point clouds through end-to-end learning. Moreover, we develop the architecture by integrating both color and geometric modalities into the point features to enhance the global descriptor representation. We conducted evaluations on public datasets ScanNet-PR and ARKit with 807 and 5047 scenarios, respectively. PoCo achieves SOTA performance: on ScanNet-PR, we achieve R@1 of 64.63%, a 5.7% improvement from the best-published result CGis (61.12%); on Arkit, we achieve R@1 of 45.12%, a 13.3% improvement from the best-published result CGis (39.82%). In addition, PoCo shows higher efficiency than CGis in inference time (1.75X-faster), and we demonstrate the effectiveness of PoCo in recognizing places within a real-world laboratory environment.

==> archives/v1.tex <==
\begin{abstract}
We present a novel algorithm (PoCo) for the Indoor RGB-D place recognition task, aimed at identifying the most likely match for a given query frame within a reference database. The task presents inherent challenges attributed to the constrained field of view and limited range of perception sensors. We propose a new network architecture, which generalizes the recent Context of Clusters (CoCs) to extract global descriptors directly from the noisy point clouds through end-to-end learning. Moreover, we integrate both color and geometric information into the point features to enhance the global descriptor representation. We conducted evaluations on public datasets ScanNet-PR and ARKit with 807 and 5047 scenarios, respectively. PoCo achieves SOTA performance: on ScanNet-PR, we achieve R@1 of $64.63\%$, a $5.7\%$ improvement from the best-published result CGis ($61.12\%$); on Arkit, we achieve R@1 of $45.12\%$, a $13.3\%$ improvement from the best-published result CGis ($39.82\%$). In addition, PoCo shows higher efficiency than CGis in inference time (2x-faster), and we demonstrate the effectiveness of PoCo in recognizing places within a real-world laboratory environment.
\end{abstract}

\section{Introduction}
% larger scope of the problem
% What is place recognition
% The high-level task is popular and necessary
For mobile robots, localization is a critical capability that enables them to determine their position within a known environment~\cite{ijcai2021p603}. Visual Place Recognition (VPR) is typically formulated as an image retrieval problem, i.e., retrieve candidate frames from a database by comparing similarities to a given query frame~\cite{lowry2015visual, ijcai2021p603}. Consequently, the design of an accurate place recognition system plays an important role in localization tasks by matching current observations with previously visited scenarios from the database~\cite{zhu2023r2former, ming2022cgis, arandjelovic2016netvlad}. It finds extensive use in applications like  navigation~\cite{stumm2013probabilistic, mirowski2018learning}, and loop closure in SLAM~\cite{bresson2017simultaneous, lowry2015visual} etc.

% different types of place recognition
Place recognition can be utilized in various environments~\cite{lowry2015visual,ijcai2021p603, zhu2023r2former,ming2022cgis}, including indoor and outdoor scenarios. Different sensors are employed based on the specific environmental conditions. For example, Lidar~\cite{uy2018pointnetvlad} and Mono-camera~\cite{zhu2023r2former,lowry2015visual} are used for outdoor place recognition, while RGB-D cameras~\cite{ming2022cgis, yudin2022hpointloc} are widely used for indoor scenarios. In this paper, our main focus is on addressing the problem of indoor RGB-D place recognition.

% smaller task, it is necessary, and its difference
While indoor and outdoor place recognition encounter similar challenges~\cite{liu2023survey, lowry2015visual}, such as varying illumination conditions, dynamic environments, and changes in view perspective, indoor place recognition possesses distinct characteristics that differentiate it from outdoor place recognition.
Firstly, indoor environments often exhibit less variability which makes it challenging to distinguish between different indoor spaces that may appear visually similar. Secondly, in indoor scenarios, RGB and depth frames often exhibit narrower field-of-view and shorter ranges compared to those of outdoor scenes~\cite{ming2022cgis}. When combined with occlusions caused by clustered objects such as furniture, clothes in daily-life settings, this results in fewer distinctive cues for recognition. Finally, Since objects in indoor scenes are typically much closer to sensors compared to those in outdoor scenes, even a slight camera motion can result in significant visual appearance changes within the field of view. Consequently, approaches tailored for outdoor scenarios may not translate effectively to indoor tasks.

\begin{figure}
    \centering    
    \includegraphics[width=\linewidth]{figs/front.png}
    \caption{As shown in the figure, the database contains several frames captured by RGB-D cameras in different rooms. The robot moves along the green trajectory and performs place recognition in real time to locate itself. When the robot moves to the red circle, it observes the blue frame and successfully finds the best-matched frame in the database.}
    \label{fig:front_page}
    \vspace{-1em}
\end{figure}

% general approach and current challenges of place recognition
% Moreover, sometimes query and database frames share small overlapping areas ~\cite{ming2022cgis, lowry2015visual}. It would cause increased false positives and severely affect the performance of navigation or SLAM applications~\cite{chen2017survey, liu2023survey}. Hence, it is desired to learn discriminative representations by combining RGB with 3D scene information.

% what other people did to solve the problem and flaws: one paragraph
A common approach for place recognition involves extracting global descriptors from both query and database frames, followed by ranking retrieved candidate frames based on the computed similarities of these global descriptors~\cite{lowry2015visual, ming2022cgis, yudin2022hpointloc}.  The recent representative work~\cite{arandjelovic2016netvlad} rely solely on color images as inputs, which demonstrate promising performance in place recognition by extending feature engineered VLAD into a data-driven learning approach. However, extracting 3D spatial geometric features from static images is still challenging. On the other hand, numerous works directly consume point clouds as their inputs. ~\cite{uy2018pointnetvlad} employs PointNet~\cite{qi2017pointnet} structure and upgrade ~\cite{arandjelovic2016netvlad} to directly extract features from a 3d point cloud. To improve the limitation of ~\cite{uy2018pointnetvlad} on capturing local geometric structures, ~\cite{komorowski2021minkloc3d} proposed to compute more discriminative 3D descriptors based on a sparse voxelized point cloud representation and sparse 3D convolutions. ~\cite{du2020dh3d} designed a Siamese network that jointly learns 3D local feature detection and description directly from raw 3D points. While point clouds offer numerous advantages such as encoded 3D spatial information and viewpoint invariance, it is arguable that integrating 3D features with 2D color features into the descriptors could potentially enhance performance further as this integration exploits the complementary nature of 3D and 2D features, leveraging the strengths of both modalities for more comprehensive scene representation. However, this research field is under explored as only few works are available for indoor RGB-D place recognition. For example, ~\cite{yudin2022hpointloc} employs Patch-NetVLAD~\cite{hausler2021patch} for image retrieval and the estimate 6 DoF camera poses based on refined feature matches with synthetic RGB-D images. The system combines various components from existing techniques and follows a piecewise optimization approach, whereas ours adopts an end-to-end learning approach. The most relevant to our work is CGiS-Net~\cite{ming2022cgis}, which aggregates both color, semantic and geometric information together using real RGB-D images, and its geometry feature is extracted by KPConv~\cite{thomas2019kpconv}. Again, CGis-Net has two distinct training stages for semantic encoder/decoder and feature encoder respectively, whereas ours is end-to-end and the network architecture is significantly different from theirs. 
% In our approach, we explicitly encode the geometric information to global descriptors by PointConvFormer~\cite{wu2023pointconvformer}. 
% As the vision transformer~\cite{liu2023survey} performs significantly well in vision tasks, 
After the Visual Transformer~\cite{dosovitskiy2021an} demonstrated promising results in various vision tasks, some transformer-based methods have been proposed, though transformers are widely recognized for their high computational cost. One most recent work R2Former~\cite{zhu2023r2former} proposed to unify global retrieval and reranking under one transformer framework. However, R2Former only works on the outdoor RGB domain. 
% Many previous RGB-based  methods~\cite{zhu2023r2former, ijcai2021p603} used transformer models for place recognition. Other approaches for indoor RGB-D place recognition use Convolution-based approaches~\cite{ming2022cgis, yudin2022hpointloc, uy2018pointnetvlad}. 
% In this project, we proposed an architecture to process the point features by transformers.

\noindent \textbf{Context of Clusters} (CoCs): CoCs~\cite{cocs} is recently introduced to efficiently extract features from RGB images. Different from transformer or convolution methods, the CoCs leverages learned centers with larger receptive field in an image to clustering and aggregate local pixels. Then it dispatches the center features to local features for further enhancement. It achieves comparable performances among other SOTA neural network architectures in multiple vision tasks. Inspired by the novel aggregation and dispatch mechanism where semantic related features will be dynamically grouped and learned together, we are attempting to apply it to enhance discriminative power of global descriptor for place recognition.  However, CoCs is only designed for 2D images, and cannot be directly applied for point clouds inference. Thus, in this paper, we are exploring to generalize this idea to jointly extracting appearance and geometric features from RGB-D data for place recognition.


% Inspired by the concept of CoCs, we extend it to indoor RGB-D place recognition tasks and propose a novel end-to-end learning neural network to process RGB-D data.

% our innovation
\textbf{Main Results:} We propose a novel architecture, as shown in Figure \ref{fig:front_page}, to handle both color appearance and geometric features from the RGB-D point cloud. We generalize CoCs to consume point clouds and make it capable of extracting both appearance and geometric features jointly from RGB-D data. 
%Our PoCo model processes geometric and RGB information to extract global descriptors for RGB-D indoor place recognition tasks. The local features of the joint color and geometric information are enhanced by a higher level of joint information of the RGB-D point cloud. 
Our approach is trained and evaluated in the ScanNet-PR~\cite{ming2022cgis} and ARKit~\cite{arkit} datasets. ScanNet-PR has 807 indoor scenarios and ARKit has 5047 scenarios, respectively. These two datasets exhibit distinct layouts, sizes, and color features across various scenarios. In particular, the ARKit dataset is collected by a mobile device, resulting in lower depth resolution and sparser RGB-D point clouds compared to ScanNet-PR. The contributions of our work include:


% We present a novel approach that directly uses RGB-D point clouds for place recognition . 
 % for feature aggregation and we propose a novel architecture based on the concept of CoCs~\cite{cocs} for global descriptor extraction. CoCs achieve similar performance in feature aggregation as the transformer~\cite{vaswani2017attention}, but offer two advantages: 1. it uses centers to enhance the local features, where the centers provide higher-level global information to the local features; 2. it has less computational cost as compared to the transformers and convolutional neural networks, and the computational efficacy is demonstrated in \cite{cocs}. 

\begin{enumerate}
    \item We propose a novel end-to-end architecture for jointly processing RGB and geometric information for indoor RGB-D place recognition. We generalize the CoCs from operating on 2D image domain to RGB-D domain, where local point features are learned by interacting with corresponding center points in a novel aggregation-and-dispatch approach.
    %Because each low-level feature does not have global information, which is the information of all features, to make the low-level features more expressive, we enhance them by global information of the point cloud. Instead of calculating all point features to get global information, we generate high-level and less number of centers with color and geometric information to enhance the low-level point features via an aggregation and dispatch mechanism. The architecture implied multiple stages to aggregate the point cloud to a single global descriptor for place recognition;
    \item We explicitly encode geometric information into the point features to enhance the representation of global descriptors for the indoor place recognition task.
    \item Our method consistently outperforms SOTA baseline models by a significant margin on multiple datasets. We observe a relative improvement of $5.7\%$ and $13\%$ in Recall@1 over baselines on ScanNet-PR~\cite{ming2022cgis} and ARKit ~\cite{arkit}, respectively.
    % We didn't use any semantic segmentation ground truth information during training.
\end{enumerate}



\section{Related Works}

% general place recognition
\textbf{Visual Place Recognition:} Place recognition is often formulated as an image retrieval problem, where the candidate frames are ranked by calculating similarities between their global descriptors and the descriptor of the query frame~\cite{ming2022cgis, zhu2023r2former}. Traditional place recognition methods extract classical RGB image features, SIFT, SURF,  etc~\cite{david2004distinctive, cummins2008fab,galvez2012bags} and use the features to compose descriptors, e.g. Bag-of-Words~\cite{sivic2008efficient}, to match the frames. SeqSLAM~\cite{milford2012seqslam} improves the accuracy by capturing the continuous geometric similarities of the features. 
% After deep learning and convolutional neural networks are proven to perform effectively in feature extraction, 
CNN-based methods~\cite{uy2018pointnetvlad, jin2017learned, gordo2017end} are widely used to process and aggregate the image features. Especially, NetVLAD-based approaches~\cite{arandjelovic2016netvlad} have resulted in higher accuracy in terms of matching for image retrieval tasks. Vision transformers~\cite{dosovitskiy2020image} are the next generation of the feature extractor and outperform CNN-based approaches in multiple tasks~\cite{touvron2021training, berton2022deep, zhu2023r2former}. In our approach, we also take advantage of transformers to process the point features.

% Indoor Place Recognition
\textbf{Indoor Place Recognition:} Different from general outdoor place recognition tasks, indoor scenes do not have a large scale. Thus, there is limited information that can be directly used~\cite{ming2022cgis}. Also because of the short range of the views, RGB-D camera~\cite{filliat2012rgbd} can be used in indoor scenarios, where the depth channel provides extra dense geometric information in this task. With RGB cameras, ORB-SLAM~\cite{rublee2011orb} uses Bag-of-Words to recognize the matching frames, and after NetVLAD place recognition method~\cite{arandjelovic2016netvlad} gets popular, FD-SLAM~\cite{yang2022fd} has been used to extract the global descriptors of frames. With RGB-D cameras, LCD~\cite{taubner2020lcd} uses the geometric information to extract the lines to help with frame matching, but they only use line features without exploiting the entire geometric information. Based on point encoding, CGiS-Net~\cite{ming2022cgis} uses KP-Conv~\cite{thomas2019kpconv} to encode the point's features and uses semantic training to pre-train the model to compute some semantic features, but it only implicitly processes the geometric information. SpoxelNet~\cite{chang2020spoxelnet} processes the global descriptor of frames by PointNet-VLAD~\cite{uy2018pointnetvlad}, which explicitly treats the geometric information as features.
%, they still use the convolution-based feature extraction method. 
% In this project, we modified~\cite{wu2023pointconvformer} to explicitly process the geometric features and also apply transformer-based architecture to extract global descriptors of points.

% Context Cluster and PointConvFormer
\textbf{Features:} Feature extraction is widely used in vision tasks~\cite{uy2018pointnetvlad,cocs,lowry2015visual}. These include classic manual-crated features~\cite{rublee2011orb, cummins2008fab} and learning-based features~\cite{arandjelovic2016netvlad, dosovitskiy2020image}.
% From the classical manual-crated features~\cite{rublee2011orb, cummins2008fab} to learning-based features~\cite{arandjelovic2016netvlad, dosovitskiy2020image}, the features become more and more representative and powerful in different vision tasks. 
Convolution-based~\cite{arandjelovic2016netvlad} and Transformer-based~\cite{zhu2023r2former} methods have been used for place recognition tasks. Recently, a new light-weighted feature extraction method Context of Clusters (CoCs)~\cite{cocs}, is proposed and demonstrates state-of-the-art performance in different vision tasks. 
% However, CoCs for now are only for RGB image processing. 
% In our work, to process the point cloud features, we apply its concept of using higher-level (lower resolution) point centers to enhance the features of the lower-level points.
% In this project, we extend the ability of the concept of context of clusters to process point features for indoor place recognition tasks. As far as we know, we are the first to apply the CoCs concept to point feature processing.

\section{Our Approach}
In this section, we first formulate the problem in Section \ref{sec:problem_formulation}, and then describe the overall architecture of our PoCo method, including our point cloud-based context cluster in Section \ref{sec:architecture}. Finally, we discuss the training strategies in Section \ref{sec:training}.

\subsection{Problem Formulation}
\label{sec:problem_formulation}

Following a similar paradigm to VPR tasks~\cite{arandjelovic2016netvlad, zhu2023r2former}, we define the indoor RGB-D place recognition task as a point cloud retrieval problem. In subsequent sections, we will refer to each frame as a colorized point cloud. Denote a query frame $\Q \in \cq$ and a candidate frame  $\D\in\cd$, where $\cq$ and $\cd$ represent query set and database respectively. In general, the model $\mathcal{M}$ transforms each frame into a global descriptor via representation learning, $\mathcal{M}: frame \rightarrow \mathbf{v} \in \mathbb{R}^n$. The goal is to retrieve likely matched candidate frames from the database based on descriptor similarities between query and database. Therefore, the model is expected to learn a representation such that positive frame pairs are close together in the embedding space, while negative frame pairs are far apart. To be more specific, $s(\mathcal{M}(\Q), \mathcal{M}(\D_p)) \gg s(\mathcal{M}(\Q), \mathcal{M}(\D_n))$ where $s(\cdot)$ is the similarity function, and $\D_p$ and $\D_n$ are positive and negative frames.

%In our approach, we use the ScanNet-PR dataset~\cite{ming2022cgis} for the place recognition task. For the training dataset, frames less than 2 meters are considered as positively matched frames and farther than 4 meters are negatively matched frames. 
% \vspace{-1em}
% \begin{align}
    
%     \label{eq:problem_definition}
% \end{align}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/architecture.png}
    \caption{\textbf{PoCo Architecture.} The inputs are the query and database RGB-D point clouds. The Feature Extractor processes the point features and generates a global descriptor for each frame. The descriptors of the query frame are compared with descriptors of the database frames by cosine similarity, and then we rank the candidate frames according to the similarities. Note that the extractor consists of Farthest Point Sampling (FPS), an encoder, and layers of Reducers and Cluster blocks (see Fig.~\ref{fig:reducer},~\ref{fig:cocs}). The FPS step processes the indices of the downsampled points at the beginning of the Feature Extractor and the following blocks sequentially apply the downsampled features.}
    \label{fig:architecture}
    \vspace{-2em}
\end{figure*}

%\subsubsection{CoCs Concept}
%CoCs process RGB image features. But its concept of feature extraction can be generalized to point clouds. CoCs models contains multiple layers for feature processing. In each layer, the image pixels are enhanced by the entire image, which is also the global information of the image. To reduce the computational cost, each CoCs layer contains two steps: Aggregation and Dispatch. 
%Aggregation uses a pooling layer to aggregate the RGB features from a large image to a smaller-dimension image. Then CoCs uses the smaller dimension image to enhance each pixel of the previous larger image. We take this concept but generalize it to processing point clouds.

\subsection{Architecture of Our PoCo Model}
\label{sec:architecture}

The architecture of our PoCo model is shown in Figure \ref{fig:architecture}. The input frames to our model possess identical tensor shapes as $N\times 9$, where $N$ is the number of points in a frame and each point is asociated with a 9-D feature vector, i.e., color $\set{r, g, b}$, position $\set{x, y, z}$ and normal $\set{n_x, n_y, n_z}$. As the Context of Clusters (CoCs)~\cite{cocs} is originally designed for 2D images, PoCo generalizes it to process 3D point cloud. In the high-level, the basic layer of the network is consisting of one Point Reducer block and one Context Cluster block. The Point Reducer downsamples point cloud and aggregate point features, while the Context Cluster enhances the point features further in an aggregation and dispatch way. To facilitate jointly learning of color and geometric features, each point feature vector is designed to have two parts: feature part and geometry part. The feature part carries the learned embedding, while geometry part stores fixed content, i.e., position and normal. The motivation to include the normal is that helps to encode points relative positional relationships for better model generalizability.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figs/place_holder.png}
%     \caption{Reducer Block}
%     \label{fig:reducer}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/pcf_cocs.png}
    \caption{\textbf{Reducer Block.} The blue circles are points in different levels. In Reducer Block, we use the Farthest Point Sampling method to downsample points and use PointConvFormer to aggregate the geometric and feature information of the K-nearest neighbors to the downsampled points. The downsampled points are also used as centers of the last layer Cluster Block to help feature processing.}
    \label{fig:reducer}
    \vspace{-1.5em}
\end{figure}

\noindent \textbf{Reducer Blocks:} Each reducer block is used to (1) downsample points population from the last layer; (2) estimate relative geometric relationships and aggregate embedding features for reduced points.  For points downsampling, we choose the Farthest Point Sampling (FPS) strategy~\cite{eldar1997farthest} for its excellent computational efficiency and ability to preserve the structure of the point cloud. Then for each point $p\in \P^{l+1}_r$, we apply KNN~\cite{kramer2013k} to choose the K nearest points from $\P^{l}_r$ as shown in Figure \ref{fig:reducer}, where $\P^{l}_r$ and $\P^{l+1}_r$ represent input and output point sets in the reducer block. The feature aggregation from $\P^l_r$ to $\P^{l+1}_r$ is based on PointConvFormer~\cite{wu2023pointconvformer} as shown in Eq.~\ref{eq:pointconvformer}, where $\cn(p)$ represents $p$'s neighbor set. $f_{1,2,3,4}(\cdot)$ are learnable Linear Layers, and $\psi(\cdot)$ is a multi-head attention module calculating the similarity score between $f(p_k)$ and $f(p)$.
% Then we apply one single PointConvFormer layer to aggregate the features from $\P^l$ and one single layer to process the features in point cloud $\P^{l+1}$.
% \vspace{-0.5em}



\begin{align}
    \f_p &= \sum_{p_k\in \cn(p)} f_4(g(p_k,p))\psi(f_1(p_k), f_2(p))f_3(p)^\top.
    \label{eq:pointconvformer}
\end{align}

% DO I NEED TO EXPLAIN MORE ABOUT THE \PSI(*)???




 The vector $g(p_k, p)$ encodes coordinate-independent geometric information as shown in Eq.\ref{eq:geos}, where $\r_k=p-p_k$ is a translation vector from $p_k$ to $p$, $\n$ and $\n_k$ are normals of $p$ and $p_k$. Thus, $g(p_k, p)$ only encodes the relative geometric information between the two points~\cite{li2021devils}.
% \vspace{-1em}
\begin{align}
    \hat{\r}_k = \frac{\r_k}{\norm{\r_k}}; \;\; &\v = \frac{\n_k-(\n_k\cdot \hat{\r}_k)\hat{\r}_k}{\norm{\n_k-(\n_k\cdot \hat{\r}_k)\hat{\r}_k}}; \;\; \w=\frac{\hat{\r}_k\times \v}{\norm{\hat{\r}_k\times \v}};\nonumber
\end{align}
 \begin{align}
    g(p_k, p) = &[\n\cdot \n_k, \frac{\r_k\cdot \n_k}{\norm{\r_k}}, \frac{\r_k\cdot \n}{\norm{\r_k}}, \n\cdot\v, \n\cdot\w, \r_k\cdot \n_k, \nonumber\\
    &\r_k\cdot(\n\times\n_k), \norm{\r_k}], 
    \label{eq:geos}
\end{align}
% couldn't find the publication version of this citation.
% After the reducer block, the features and geometric information would be sent to the following Context Cluster blocks.



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/cluster.png}
    \caption{\textbf{Cluster Block.} Red points are centers downsampled from the blue points. The blue points are grouped by the similarity of w.r.t. the red centers. Then the features of the blue points are aggregated to the centers by Eq.~\ref{eq:cluster} and then the center features are dispatched to the points by Eq.~\ref{eq:dispatch}.}
    \label{fig:cocs}
    \vspace{-2em}
\end{figure}
\noindent\textbf{Context Cluster Blocks:} Points in the block are dynamically clustered into groups/centers based on their learned affinities in the embedding space during the aggregation stage. As semantically correlated point features are more likely to be grouped together, each center point can effectively learn richer features from its associated member points. After that, aggragated center features will be adaptively dispatched to each member point based on the similarity. In this way, member points implicitly communicate with each other via their center point and learn to optimize features jointly. We provide an overview of context cluster in Fig.\ref{fig:cocs} and will delve into further details in the following sections.

\textbf{Aggregation:} For the point set $\P^{l+1}_r$, we downsample it to generate center points $\P^{l+1}_c$, where the cardinality $\abs{\P^{l+1}_r} = N_r > \abs{\P^{l+1}_c} = N_c$. Each center feature $\f_c$ is initialized as the mean vector of its K spatially nearest point features $\{\f_p\}$ from $\P^{l+1}_r$. As is shown in Fig.~\ref{fig:cocs},in the aggregation stage, we firstly calculate the cosine similarity scores between all the centers and all the points: $s_{c,p} = \sigma(\alpha \cdot cosine(\f_p, \f_c)+\beta)$, where $\sigma(\cdot)$ is the sigmoid activation function and $\alpha$ and $\beta$ are trainable parameters. Then point features are aggregated into center points according to previous computed similarities. The center feature $\f_c$ is incorporated as an anchor feature for numerical stability as well as further emphasize the locality in Eq. \ref{eq:cluster}
\begin{align}
    \f_c = \frac{1}{\cc} \left( \f_c + \sum_{p=1}^{N_r}  \s_{c,p} \cdot \f_p \right),
    \label{eq:cluster}
\end{align}
$\cc=1+\sum_{p=1}^N \s_{c,p}$, is the normalization factor.

\textbf{Dispatch:} The previous learned similarities are used to dispatch the aggregated center features to their member cluster points via Eq.\ref{eq:dispatch}:
\vspace{-0.5em}
\begin{align}
    \f_p = \f_p + h(s_{c,p} \cdot \f_c )).
    \label{eq:dispatch}
\end{align}
%The Context Cluster block uses \textbf{all centers} of the point cloud to enhance each point feature of the point $p\in\P^l$. So this process provides the global information of the point clouds to each point $p$.
% In this way, we generalized the concept of Context Clusters~\cite{cocs} to process the point cloud features, which was not handled by ~\cite{cocs}.

\textbf{Global Descriptor Extraction:} The Encoder shown in Figure \ref{fig:architecture} aggregates all the point features from the last Context Cluster block into a global descriptor, which is used to measure the similarity between the query frame and candidate frames of database. We adopt cosine similarity as the metric function. The encoder is implemented as a variant of the Reducer Block, which is configured to have a single point as the output. Its input point features are all normalized and aggregated by the geometric and feature weights as described in Equation \ref{eq:pointconvformer}. In the experiments, the dimension of the global descriptor is set to 256. 

\subsection{Training}
\label{sec:training}

% Traditionally, place recognition methods train the models by telling the difference between positive and negative cases with Triplet loss. In PoCo, we also want the training to estimate the 
% Previous place recognition tasks only rank the candidate frames without calculating the similarity score between the candidate frames and the query frame (with global descriptor $\g_q$). In comparison, PoCo recognises the difference between positively matched frames (with global descriptor $\g_p$) and negatively matched frames (with global descriptor $\g_n$) and also computes the difference scores between each query-candidate pair. 

During training, models are optimized to distinguish positive examples from negative examples. We utilize the widely used Triplet Loss~\cite{schroff2015facenet} for this purpose. In addition to distinguishing differences, we aim to provide guidance to estimate the similarity within certain boundaries for stable training. Therefore, Circle Loss is also employed in the training loss~\cite{sun2020circle}.

% This function is achieved by using both Circle Loss~\cite{sun2020circle} and Triplet Loss~\cite{schroff2015facenet}. 
The circle loss, $\cl_c$, is defined as Equation~\ref{eq:circle}. $m=0.2$ is the margin to reinforce the optimization. $cl(\cdot)$ is a clamp function, which clamp the value to 0 if it is negative.  $\gamma=1$ is a hyperparameter. $s_p$ and $s_n$ are cosine similarities of  the query-positive frame pair and query-negative frame pair, respectively. The circle loss is to guide the similarities between the query and positive cases to 1 and negative cases to 0.
\begin{align}
    a_p = cl(s_p-1-m, 0), a_n = cl(s_n+m, 0) \\
    \cl_c = softplus(\log \sum \exp(\gamma a_n (s_n - \delta_n)) - \\
    \log \sum \exp(\gamma a_p (s_p - \delta_p)))
    \label{eq:circle}
\end{align}

% In Equation \ref{eq:circle}, $softplus(\cdot)$ is the soft plus function. Function $cl(\cdot)$ represents the clamp minimum, where the value is clamped by 0. The $m=0.2$ is the margin. $\gamma=1$ is a hyperparameter. $s_p$ and $s_n$ are similarities between the query frame and the matched frames and not matched frames, respectively, and the similarity is calculated by cosine similarity between the global descriptors.

Triplet loss, $\cl_t$, is defined as Equation \ref{eq:triplet}. Triplet loss is to maximize the difference between the distances of the query-positive frame pair and query-negative frame pair. The distance between the query and database descriptors is calculated by the L2 distance function $d(\cdot, \cdot)$. The margin is set as $m=0.2$.

% As Equation \ref{eq:triplet}, triplet loss, $\cl_t$, uses L2 distance, $d(\cdot)$, to calculate the distances between global descriptors of query frame and database frame. $m=0.2$ is the margin.

\begin{align}
    \cl_t = \max(d(\g_p, \g_q) - d(\g_n, \g_q) + m, 0)
    \label{eq:triplet}
\end{align}

In the final loss function, we combine the two losses $\cl = \alpha \cl_c + \beta \cl_t$. In experiments, we find the best weights for these two terms as $\alpha=10$ and $\beta=0.1$ via hyper-parameters tuning. By assigning a higher weight to triplet loss, the model can rapidly converge to a specific range, facilitating the differentiation between positive and negative examples. Subsequently, circle loss aids in refining the estimation process, resulting in more accurate similarity values that closely align with the boundaries.

% During training, the candidate is mostly ranked by the similarity of the candidate frames so computing the difference between matched frames and not matched frames is the most important, therefore, the triplet loss is the major loss. We give a large weight to triplet loss, $\alpha=10$, and a smaller weight to circle loss, $\beta=0.1$.

\section{Experiments}
In this section, we introduce two large-scale datasets with various challenging scenarios for training and evaluation. Then we describe the settings of the implementation. For evaluations, considering our problem is \textbf{indoor RGB-D point cloud place recognition}, first we show our approach outperforms other SOTA indoor point-cloud-based approaches in the two datasets with both quantitative and qualitative results, and then we also use ablation studies to show the capability of our model in processing both color and geometric information for indoor RGB-D place recognition tasks.

\subsection{Dataset and Training Settings}

Our approach is trained and evaluated on two indoor RGB-D datasets, ScanNet-PR~\cite{ming2022cgis} and ARKit~\cite{arkit}. These two datasets are all large datasets for learning purposes and have various object features, sensors, and illumination conditions. ScanNet-PR is derived from the ScanNet dataset~\cite{dai2017scannet} captured by RGB-D cameras and ARKit is captured by an iPad camera and a dense Lidar sensor. In evaluation, we show that our approach outperforms other state-of-the-art approaches in the challenging datasets. The datasets contain lots of scenarios, and each scenario represents a room with multiple frames. Each frame contains a point cloud with both colors ($\set{r, g, b}$) and geometric ($\set{x, y, z}$) information for each point, but for different frames the numbers of points are different. ScanNet-PR has 807 scenarios in total and is split into training (565), validation (142), and testing (100) datasets. For the ARKit dataset, we use a similar strategy as ScanNet-PR~\cite{ming2022cgis} to process the ARKit dataset~\cite{arkit}. The ARKit dataset has 5047 scenarios and we separate it into training (3958), validation (1089), and testing (100) datasets. 

Our PoCo model is implemented by Pytoch and trained on 8 Tesla-V100 GPUs. The input points are constrained to 2000 points by voxelization. Besides $\set{r, g, b}$ and $\set{x, y, z}$ information, we also use the normal vectors $\set{n_x, n_y, n_z}$ of each point to provide relative geometric information as Equation~\ref{eq:geos}, which is calculated by the plane within a 0.2-meter radius of the point. For the training strategy, we use cosine annealing scheduler~\cite{loshchilov2016sgdr} with Adam optimizer~\cite{kingma2014adam}. The increase factor of the scheduler is $1$ and learning rate starts from $10^{-4}$ to $10^{-7}$. 

\subsection{Implementations of Comparison and Ablation Study}
To make a fair comparison, we use the SOTA evaluation strategy of CGiS-Net~\cite{ming2022cgis}, which is the current best approach in the ScanNet-PR dataset. In each scenario of the datasets, the keyframes are chosen by a distance threshold of 3 meters, and other frames are query frames. For each query frame, we use the Recall metric to evaluate the place recognition performance: The similarities between the query frame and the keyframes from \textbf{all testing scenarios in the dataset} are calculated and the keyframes are ranked by the similarity. The Recall@k represents the accuracy of the k$_{th}$ candidate as a matched frame to the query.  Besides Recall@k, we also evaluate the running time (inference time), FLOPs, and model size of different approaches. All the metrics are evaluated in the device with one NVIDIA GeForce RTX 3060 GPU and an Intel Xeon(R) W-2255 CPU. 


To evaluate the performance of our approach, PoCo, we compare with different SOTA indoor RGB-D point cloud-based place recognition approaches, CGiS-Net~\cite{ming2022cgis}, MinkLoc-3D~\cite{komorowski2021minkloc3d}, NetVLAD~\cite{arandjelovic2016netvlad}, PointNet-VLAD~\cite{uy2018pointnetvlad}, Indoor DH3D~\cite{du2020dh3d}, SIFT feature with Bag of Words~\cite{sivic2008efficient}. All these approaches are trained and tested in the two datasets, separately. 

For the ablation study, to demonstrate the capability of our model in handling both color and geometric information, we designed three types of experiments: 1. Vanilla RGB CoCs, which uses the CoC-Medium~\cite{cocs} as the backbone and applied our Encoder block of Figure~\ref{fig:architecture}. This is to test the capability of CoCs in RGB place recognition, and also shows how much effect color information takes in place recognition task; 2. PoCo w/o Color, which only processes geometric information of the point cloud, where the input feature changes from $\set{r,g,b,x,y,z}$ to $\set{x,y,z}$. This ablation study tests the efficacy of our PoCo model using geometric information in place recognition tasks; 3. PoCo w/o Equation \ref{eq:geos}, which removes the relative geometric information and the model only uses absolute positions of the points. This model is to test how much effect the relative geometric function has on the place recognition performance.

% In our implementation, besides the complete PoCo model, we also designed a Vanilla RGB model based on the CoCs feature extractor. We use the CoC-Medium~\cite{cocs} as the backbone and in the last layer, we apply another reducer, where we apply a 2D-convolutional layer to the centers from the last layer of CoC-Medium and output a global descriptor with the dimension of 256. Another model for ablation study is the PoCo w/o color, where we only use coordinates and normals as the input feature of each point and process the features by our PoCo architecture. 

% CGiS-Net is the baseline method to compare with. We are following the same experiment setup as CGis-Net work. To be specific, the recall values are calculated on the testing dataset, where the candidate point clouds are chosen by a distance threshold of 3 meters. 

% Given a query frame, we calculate the similarities of the candidate global descriptors with the descriptor of the query frame and then rank the candidate frames according to the similarity. The standard evaluation metric Recall @ K is calculated by the percentage of correctly matched query frames given to top K candidates. Besides CGiS-Net, we also compared with NetVLAD~\cite{arandjelovic2016netvlad}, PointNetVLAD~\cite{uy2018pointnetvlad}, Indoor DH3D~\cite{du2020dh3d} and MinkLoc3D~\cite{komorowski2021minkloc3d}. We present the quantitative results (recall@K) on the ScanNet-PR dataset in Table \ref{tab:recall_scannet} and \ref{tab:recall_arkit} and show qualitative comparisons from different room environments.





\begin{table}[h!]
    \centering
    \begin{tabular}{c|c|c|c}
ScanNetPR & R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$\\
\hline
SIFT~\cite{david2004distinctive} + BoW~\cite{sivic2008efficient} & 16.16 & 21.17 & 24.38 \\
\hline
NetVLAD~\cite{arandjelovic2016netvlad} & 21.77 & 33.81 & 41.49 \\
\hline
PointNet-VLAD~\cite{uy2018pointnetvlad} & 22.43 & 30.81 & 36.58 \\
\hline
Indoor DH3D~\cite{du2020dh3d} & 16.10 & 21.92 & 25.30 \\
\hline
MinkLoc-3D~\cite{komorowski2021minkloc3d} & 10.13 & 16.63 & 20.80 \\
\hline
CGiS-Net~\cite{ming2022cgis} & 61.12 & 70.23 & 75.06 \\
\hline
CGiS-Net w/o color~\cite{ming2022cgis} & 39.62 & 50.92 & 56.14 \\
\hline
CGiS-Net w/o geometry~\cite{ming2022cgis} & 40.07 & 51.28 & 58.96 \\
\hline
\hline
Vanilla RGB CoCs~\cite{cocs} & 41.82 & 57.65 & 66.82 \\
\hline
PoCo w/o color & 44.34 & 54.27 & 59.78 \\
\hline
PoCo w/o Equation~\ref{eq:geos} & 62.23 & 73.81 & 79.63 \\
\hline
PoCo & \textbf{64.63} & \textbf{75.02} & \textbf{80.09} \\
    \end{tabular}
    \caption{The table shows our PoCo method outperforms other state-of-the-art methods by at least $5.7\%$ improvement in Recall@1 value in the ScanNetPR dataset.} 
    \label{tab:recall_scannet}
    \vspace{-1em}
\end{table}


% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c}
% ScanNetPR & R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$\\
% \hline
% CGiS-Net~\cite{ming2022cgis} & 61.12 & 70.23 & 75.06 \\
% \hline
% CGiS-Net w/o color~\cite{ming2022cgis} & 39.62 & 50.92 & 56.14 \\
% \hline
% CGiS-Net w/o geometry~\cite{ming2022cgis} & 40.07 & 51.28 & 58.96 \\
% \hline
% \hline
% Vanilla RGB CoCs~\cite{cocs} & 41.82 & 57.65 & 66.82 \\
% \hline
% PoCo w/o color & 44.34 & 54.27 & 59.78 \\
% \hline
% PoCo w/o Equation~\ref{eq:geos} & 62.23 & 73.81 & 79.63 \\
% \hline
% PoCo & \textbf{64.63} & \textbf{75.02} & \textbf{80.09} \\
%     \end{tabular}
%     \caption{The table shows our PoCo method outperforms baseline models w.r.t recall @ K in the ScanNetPR dataset. For R@1, our Vanilla RGB outperforms the CGiS-Net w/o geometry around $2\%$ and our PoCo w/o color outperforms CGiS-Net w/o color around $5\%$. It is worth highlighting that being different from CGis-Net, PoCo doesn't use any semantic segmentation ground truth labels in our training stage.}
%     \label{tab:recall_scannet_ablation}
% \end{table}

\begin{table}[h!]
    \centering
    \begin{tabular}{c|c|c|c}
ARKit & R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$\\
\hline
PointNet-VLAD~\cite{uy2018pointnetvlad} & 11.04 & 16.57 & 20.57 \\
\hline
MinkLoc-3D~\cite{komorowski2021minkloc3d} & 8.14 & 10.95 & 13.79 \\
\hline
CGiS-Net~\cite{ming2022cgis} & 39.82 & 49.01 & 56.02 \\
\hline
\hline
Vanilla RGB CoCs~\cite{cocs} & 17.19 & 24.74 & 30.06 \\
\hline
PoCo w/o color & 21.58 & 30.00 & 35.66 \\
\hline
PoCo w/o Equation~\ref{eq:geos} & 41.41 & 51.86 & 58.11 \\
\hline
PoCo & \textbf{45.12} & \textbf{57.10} & \textbf{62.14} \\
    \end{tabular}
    \caption{The table shows our PoCo model outperforms other approaches by at least 4 in Recall@1 in the ARKit dataset. Our PoCo model is much better than other approaches even without the relative geometric information, and this indicates the feature processor are capable of encoding enough local and global information of the frame in the global descriptor.} 
    \label{tab:recall_arkit}
    \vspace{-1em}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c|c}
\multirow{ 2}{*}{Methods} & \multirow{ 2}{*}{R@1$\uparrow$} &  Running &  FLOPs & Model \\
 & &   Time (s) & (Mb)  &  Size (Mb)\\ \hline
 PointNet-VLAD & 22.43 & 0.01 & 1319.67 & 75.47 \\ \hline
 MinkLoc-3D & 10.13 &0.02 & - & 10.17 \\ \hline
 CGiS-Net & 61.12 & 0.07 & 738.60 & 26.18 \\ \hline
 PoCo & 64.63 & 0.04 & 285.63 & 29.94 \\ \hline
    \end{tabular}
    \caption{Our approach is 2X faster than CGiS-Net and also has better recall values. Our computational cost is the smallest compared with other approaches.} 
    \label{tab:computation}
    \vspace{-1em}
\end{table}


\subsection{Results}
In Table \ref{tab:recall_scannet} and Table \ref{tab:recall_arkit}, we evaluate the performance of different SOTA approaches compared with our PoCo method and also ablation studies in two datasets. From Table \ref{tab:recall_scannet}, the learning-based methods show better accuracy in Recall@1 than SIFT+BoW. In the ScanNetPR dataset (Table \ref{tab:recall_scannet}), our PoCo method outperforms the other approaches by at least $5.7\%$  in Recall@1 and In the ARKit dataset (Table \ref{tab:recall_arkit}) we have at least $4$ points improvement. Considering PointNet-VLAD and MinkLoc-3D only process geometric information, in Table \ref{tab:recall_scannet}, we compare PoCo w/o color with these two methods and CGiS-Net w/o color. Our pure geometric model still outperforms other approaches by at least $11.91\%$ in Recall@1. In the ARKit dataset, our PoCo w/o color also outperforms other pure-geometric methods. The result means our model can effectively process geometric information in indoor RGB-D place recognition tasks and proofs the efficacy of our innovations in generalizing CoCs concept to point clouds. From Figure~\ref{fig:qualitative_results_scannet} and Figure~\ref{fig:qualitative_results_arkit}, we observe our model is much better than other approaches in the challenging cases, where the overlap (red-circled) areas between query and positive frames are very small. From These two figures, we can also observe that PointNet-VLAD cannot recognize different colors for matching, whereas, in Figure~\ref{fig:qualitative_results_scannet}, it chooses a scenario with a completely different color as the best match. Besides the accuracy, as shown in Table \ref{tab:computation}, we also compared the computational cost of different approaches. Compared with CGiS-Net, our PoCo model achieves both higher accuracy in Recall and less computational cost. The PointNet-VLAD and MinkLoc-3D have less inference time, but their accuracy is much worse than our model. %Because PoCo w/o color only changes input dimension from 6 to 3 in the first layer, the running time and FLOPs are mostly the same as PoCo.

About Ablation studies, as shown in Table \ref{tab:recall_scannet} and Table \ref{tab:recall_arkit}, geometric information and color information are both important to place recognition and they have very similar effects on the Recall values. Geometric information matters more than color information, and by only using each of them, in Table~\ref{tab:recall_scannet} PoCo w/o color has Recall@1 $2.52$ higher than the RGB model. In Table~\ref{tab:recall_arkit}, it has a larger difference of $4.39$, which means that our design can effectively process geometric information for place recognition. Comparing Poco with PoCo w/o Equation~\ref{eq:geos}, we observe that relative geometric information makes the method more generalized to different point clouds and achieves 2.4 and 3.71 improvement in Recall@1 in ScanNetPR and ARKit datasets, respectively. Figure \ref{fig:color_results} provides the qualitative difference between PoCo and RGB models. RGB model can only detect similar objects, but cannot tell complex positional relations among the object. Compared with it, our PoCo method can both recognize the objects and their relative positions in the scenarios. From Figure~\ref{fig:geometric_results}, PoCo w/o Color is capable of recognizing very similar structures, such as the table and the chair in the first row. But because it doesn't have color information, it falsely matched the frames with very obvious color differences. However, PoCo is capable of utilizing color information to find the best match. From the ablation study, we demonstrate the efficacy of our innovation in jointly processing different modalities, color and geometric information, and achieves higher accuracy in indoor RGB-D place recognition tasks.


\input{qualitative}

% \subsection{Recall Values}
% We evaluate the performance of our method by comparing with baseline methods, CGiS-Net~\cite{ming2022cgis}, MinkLoc-3D~\cite{komorowski2021minkloc3d}, DH3D~\cite{du2020dh3d}, PointNet-VLAD~\cite{uy2018pointnetvlad}, NetVLAD~\cite{arandjelovic2016netvlad} and SIFT feature with Bag of Words~\cite{sivic2008efficient}. As shown in Table \ref{tab:recall_scannet}, our full PoCo model outperforms the other approaches by at least $5.7\%$. We also evaluate the effect of different types of features on the final results, as shown in Table \ref{tab:recall_scannet_ablation}, and we apply the ablation studies by using only RGB color features and only geometric features. Our PoCo model w/o color achieves around $5\%$ improvement compared with CGiS-Net w/o color and the PoCo model w/o geometry outperforms CGiS-Net w/o geometry by around $2\%$. The results mean not only can our model effectively embed the geometric information of the point cloud, but also process color features better than the other state-of-the-art method. From the table, we can also notice that the PoCo w/o color is better than PoCo w/o geometric, which means geometric information plays an important role in the place recognition task. To demonstrate the effects of the relative geometric information compared with absolute points positional information, we remove Equation~\ref{eq:geos} and only use points absolute positions, as PoCo w/o Equation~\ref{eq:geos} in Table \ref{tab:recall_scannet_ablation} . As shown in Table \ref{tab:recall_scannet_ablation}, using relative geometric information can improve the recall@1 value around 2.

% We also compared our approach with PointNet-VLAD~\cite{uy2018pointnetvlad}, MinkLoc-3D~\cite{komorowski2021minkloc3d} and CGis-Net~\cite{ming2022cgis} in ARKit dataset. As shown in Table \ref{tab:recall_arkit}, our PoCo model also outperforms other approaches in ARKit dataset by at least \textbf{$13\%$} in Recall@1. Considering the points in ARKit are sparser than ScanNetPR, the recall values are relatively lower than those in ScanNetPR.









% \subsection{Qualitative Results}
% In this section, we show the comparisons between our approach and the CGiS-Net in qualitative pictures and we also evaluate how geometric and color information affect the performance. 

% As shown in Figure \ref{fig:qualitative_results_scannet} and \ref{fig:qualitative_results_arkit} of both ScanNetPR and ARKit datasets, our PoCo model can find the best-matched frames even though the overlap area is very small, as the red circles marked in the figure. Figure \ref{fig:geometric_results} shows how geometric information helps in the place recognition task. As shown in Figure \ref{fig:geometric_results}, the Vanilla-RGB-PR model can detect objects, such as chairs and washing machines, but it cannot recognize the relative positions of the objects very well. The complete PoCo model can effectively handle the geometric relations of the objects in the scenarios. Figure \ref{fig:color_results} shows the comparison between the complete PoCo and PoCo w/o Color, where only geometric information is used in the model. As shown in the figure, we can see the PoCo w/o Color is capable of recognizing very similar structures, such as the table and the chair in the first row, and the bed in the second row. But because it doesn't have color information, it falsely matched the frames with very obvious color differences. The complete PoCo model can effectively combine the color and geometric information in the recognition task.



\section{Conclusion, Limitations and Future Work}
We are the first to propose a Point-Cloud-based place recognition model based on the concept of CoCs. We explicitly encode geometric information during feature extraction with transformer-based models. PoCo outperforms previous indoor RGB-D place recognition methods significantly in recall@K. However, our model still has its limitations, where sometimes our model relies much on geometric information which hurts the performance, and in some extreme cases, the overlapping areas between the ground truth and query frame are small and do not have many features. To solve the issues, we could use local features to help re-ranking candidate frames to improve accuracy. Therefore, in the future, a second stage of re-ranking candidates will be explored.

% \section*{ACKNOWLEDGMENT}


==> archives/v1_ICRA.tex <==
\begin{abstract}
We present a novel algorithm (PoCo) for Indoor RGBD place recognition task, where the goal is to identify the most probable match for a given query frame from a reference database. We address many challenges related to limited field of view and range of perception sensors, and present a new Point Cloud-based Context Cluster method to extract appropriate features from the point cloud using an  end-to-end learning network.  These features are  used to generate a global description of a frame for place recognition. Moreover, we encode geometric information into the point features to enhance the representation of global descriptors for the indoor place recognition task. We evaluate the performance on the public ScanNet-PR data, which has 807 scenarios with very different layouts. We observe that our PoCo model significantly outperforms state-of-the-art methods by at least $5.7\%$ with respect to standard recall@K metric. We show that this method effectively recognize places in a real-world lab environment.
\end{abstract}

\section{INTRODUCTION}
% larger scope of the problem
% What is place recognition
% The high-level task is popular and necessary
For mobile robots, localization is an essential capability, which enables a robot to find its position in a known environment~\cite{ijcai2021p603}. Visual place recognition tasks are usually formulated as an image retrieval problem, which is to retrieve candidate frames from a database by a given query frame~\cite{lowry2015visual, ijcai2021p603}.  Thus, place recognition plays an important role in the localization task by matching the current observation with previous visited scenarios from the database~\cite{zhu2023r2former, ming2022cgis, arandjelovic2016netvlad}. It is used in many applications such as navigation~\cite{stumm2013probabilistic, mirowski2018learning}, and SLAM~\cite{bresson2017simultaneous, lowry2015visual} etc. Thus, designing an accurate place recognition system is important for robotics and navigation applications.

% different types of place recognition
Place recognition can be used in different environments~\cite{lowry2015visual,ijcai2021p603, zhu2023r2former,ming2022cgis}, e.g., indoor and outdoor scenarios. Different sensors are adopted for different scenarios. For example, Lidar~\cite{uy2018pointnetvlad} and Mono-camera~\cite{zhu2023r2former,lowry2015visual} are used for outdoor place recognition. For indoor scenrios, RGBD cameras~\cite{ming2022cgis, yudin2022hpointloc} are widely used. In this paper, we mainly address the problem of indoor RGBD place recognition.

% smaller task, it is necessary, and its difference
Though indoor place recognition shares similar goals with outdoor one, it has its own characteristics. Thus, approaches designed for outdoor scenarios may not work well for indoor tasks. For example, RGB and depth frames in indoor scenarios may have narrower field of views and shorter ranges compared with outdoor scenes, which makes it  challenging for matching~\cite{ming2022cgis}. As long-range perception is not required in indoor place recognition, RGBD cameras are well-suited to it. Depth maps can also provide dense geometric information that is complementary to RGB information. 

\begin{figure}
    \centering    
    \includegraphics[width=\linewidth]{figs/front.png}
    \caption{As shown in the figure, the database contains several frames captured by RGBD camera in different rooms. The robot moves along the green trajectory and perform place recognition in real time to locate itself. When the robot moves to the red circle, it observes the blue frame and successfully find the best-matched frame in the database.}
    \label{fig:front_page}
    \vspace{-1em}
\end{figure}

% general approach and current challenges of place recognition
Place recognition has many challenges~\cite{liu2023survey, lowry2015visual}, including varying illumination conditions, dynamic environments, view perspective changes etc. Since objects in indoor scenes are typically much closer to sensors as compared to those in outdoor scenes, a small motion of the camera can lead to significant visual appearance changes in the field of view. Thus, learning view-invariant features leveraging the 3D structure of the scene is desired. Moreover, sometimes query and database frames share small overlapping areas ~\cite{ming2022cgis, lowry2015visual}. It would cause increased false positives and severely affect performance of navigation or SLAM applications~\cite{chen2017survey, liu2023survey}. Hence, it is desired to learn discriminative representations by combining RGB with 3D scene information.

% what other people did to solve the problem and flaws: one paragraph
A general approach for place recognition is to extract global descriptors of both query and database frames, and then rank retrieved candidate frames based on comparing the similarities computed from those global descriptors~\cite{lowry2015visual, ming2022cgis, yudin2022hpointloc}.  Some of current place recognition methods~\cite{arandjelovic2016netvlad, zhu2023r2former} only use RGB information that don't encode any geometric information in the descriptors. CGiS-Net~\cite{ming2022cgis} uses geometric information, but only implicitly processes it by KPConv~\cite{thomas2019kpconv}. 
% In our approach, we explicitly encode the geometric information to global descriptors by PointConvFormer~\cite{wu2023pointconvformer}. 
% As the vision transformer~\cite{liu2023survey} performs significantly well in vision tasks, 
Many previous RGB-based  methods~\cite{zhu2023r2former, ijcai2021p603} used transformer models for place recognition. Other approaches for indoor RGBD place recognition use Convolution-based approaches~\cite{ming2022cgis, yudin2022hpointloc, uy2018pointnetvlad}. 
% In this project, we proposed an architecture to process the point features by transformers.

The concept of Context of Clusters (CoCs): CoCs method~\cite{cocs} works efficiently on feature extraction. Instead of calculating the same level pixel features as the transformer or convolution methods, the CoCs method finds higher-level centers in an image to aggregate the nearby local pixels. Then it dispatches the center features to local features for further enhancement. This method is used to perform more efficient feature computation for image processing and also achieves comparable performances among other SOTA neural network architectures in multiple vision tasks and computer vision~\cite{cocs}. 
% Inspired by the concept of CoCs, we extend it to indoor RGBD place recognition task and propose a novel end-to-end learning neural network to process RGBD data.

% our innovation
\textbf{Main Results:}  We present a new approach that directly uses RGBD point clouds for place recognition as shown in Figure \ref{fig:front_page}. Our PoCo model takes advantage of the geometric information of points and also applies the concept of CoCs~\cite{cocs} to a transformer-based architecture for global descriptor extraction. Our approach based on CoCs achieves similar feature aggregation as the transformer~\cite{vaswani2017attention}, but offers two advantages: 1. it uses global centers to enhance the local features, where the centers provide higher-level information to the local features; 2. it has less computational cost as compared to the transformers and convolutional neural networks. This approach is trained and evaluated in the ScanNet-PR dataset~\cite{ming2022cgis}, which has 807 indoor scenarios with very different layout, sizes, and color features. Some of the novel aspects of our work include:
\begin{enumerate}
    \item We present a novel end-to-end learning network for point cloud feature extraction based on the concept of Context of Clusters, where point features are learned by propagating/exchanging info via feature clustering centers in an aggregation and dispatch mechanism. The processed features are used to generate a global descriptor of a frame for place recognition;
    \item We explicitly encode geometric information into the point features to enhance the representation of global descriptors for the indoor place recognition task;
    \item In ScanNet-PR~\cite{ming2022cgis} dataset, we compared our method with SOTA baseline models such as CGiS-Net~\cite{ming2022cgis}, NetVLAD~\cite{arandjelovic2016netvlad}, MinkLoc~\cite{komorowski2021minkloc3d} etc. We observe relative improvement of $5.7\%$ in recall scores on place recognition tasks. 
    % We didn't use any semantic segmentation ground truth information during training.
\end{enumerate}



\section{Related Works}

% general place recognition
\textbf{Visual Place Recognition:} Place recognition is often formulated as an image retrieval problem, where the candidate frames are ranked by calculating similarities between their global descriptors and the descriptor of the query frame~\cite{ming2022cgis, zhu2023r2former}. Traditional place recognition methods extract classical RGB image features, SIFT, SURF,  etc~\cite{david2004distinctive, cummins2008fab,galvez2012bags} and use the features to compose descriptors, e.g. Bag-of-Words~\cite{sivic2008efficient}, to match the frames. SeqSLAM~\cite{milford2012seqslam} improves the accuracy by capturing the continuous geometric similarities of the features. 
% After deep learning and convolutional neural networks are proven to perform effectively in feature extraction, 
CNN-based methods~\cite{uy2018pointnetvlad, jin2017learned, gordo2017end} are widely used to process and aggregate the image features. Especially, NetVLAD-based approaches~\cite{arandjelovic2016netvlad}  has resulted in higher accuracy in terms of matching for image retrieval tasks. Vision transformers~\cite{dosovitskiy2020image} are the next generation of the feature extractor and outperform CNN-based approaches in multiple tasks~\cite{touvron2021training, berton2022deep, zhu2023r2former}. In our approach, we also take advantage of transformers to process the point features.

% Indoor Place Recognition
\textbf{Indoor Place Recognition:} Different from general outdoor place recognition tasks, indoor scenes do not have a large scale. Thus, there is limited information that can be directly used~\cite{ming2022cgis}. Also because of the short range of the views, RGBD camera~\cite{filliat2012rgbd} can be used in indoor scenarios, where the depth channel provides extra dense geometric information in this task. With RGB cameras, ORB-SLAM~\cite{rublee2011orb} uses Bag-of-Words to recognize the matching frames, and after NetVLAD place recognition method~\cite{arandjelovic2016netvlad} gets popular, FD-SLAM~\cite{yang2022fd} has been used to extract the global descriptors of frames. With RGBD cameras, LCD~\cite{taubner2020lcd} uses the geometric information to extract the lines to help with frame matching, but they only use line features without exploiting the entire geometric information. Based on point encoding, CGiS-Net~\cite{ming2022cgis} uses KP-Conv~\cite{thomas2019kpconv} to encode the point's features and uses semantic training to pre-train the model to compute some semantic features, but it only implicitly processes the geometric information. SpoxelNet~\cite{chang2020spoxelnet} processes the global descriptor of frames by PointNetVLAD~\cite{uy2018pointnetvlad}, which explicitly treats the geometric information as features.
%, they still use the convolution-based feature extraction method. 
% In this project, we modified~\cite{wu2023pointconvformer} to explicitly process the geometric features and also apply transformer-based architecture to extract global descriptors of points.

% Context Cluster and PointConvFormer
\textbf{Features:} Feature extraction is widely used in vision tasks~\cite{uy2018pointnetvlad,cocs,lowry2015visual}. These include classic manual-crated features~\cite{rublee2011orb, cummins2008fab} and learning-based features~\cite{arandjelovic2016netvlad, dosovitskiy2020image}.
% From the classical manual-crated features~\cite{rublee2011orb, cummins2008fab} to learning-based features~\cite{arandjelovic2016netvlad, dosovitskiy2020image}, the features become more and more representative and powerful in different vision tasks. 
Convolution-based~\cite{arandjelovic2016netvlad} and Transformer-based~\cite{zhu2023r2former} methods have been used for place recognition tasks. Recently, a new light-weighted feature extraction method Context of Clusters (CoCs)~\cite{cocs}, is proposed and demonstrates state-of-the-art performance in different vision tasks. 
% However, CoCs for now are only for RGB image processing. 
% In our work, to process the point cloud features, we apply its concept of using higher-level (lower resolution) point centers to enhance the features of the lower-level points.
% In this project, we extend the ability of the concept of context of clusters to process point features for indoor place recognition tasks. As far as we know, we are the first to apply the CoCs concept to point feature processing.

\section{Our Approach}
In this section, we first formulate the problem in Section \ref{sec:problem_formulation}, and then describe the overall architecture of our PoCo method, including our point cloud-based context cluster in Section \ref{sec:architecture}. Finally, we discuss the training strategies in Section \ref{sec:training}.

\subsection{Problem Formulation}
\label{sec:problem_formulation}

Similar to other visual place recognition tasks~\cite{arandjelovic2016netvlad, zhu2023r2former}, we define the indoor RGBD place recognition task as a point cloud retrieval problem. Denote a query RGBD point cloud $\P_i \in \cp_q$ and a database of RGBD point cloud $\cq_d$, where $\cp_q$ and $\cq_d$ are point cloud sets including multiple cloud frames. Each point cloud can extract one global descriptor. By comparing the descriptor of the query point cloud with descriptors of the database, the indoor RGBD place recognition task calculates the most similar candidates of the query point cloud from the database. In our approach, we use the ScanNet-PR dataset~\cite{ming2022cgis} for the place recognition task. For the training dataset, frames less than 2 meters are considered as positively matched frames and farther than 4 meters are negatively matched frames. The target of this method is to distinguish the positive and negative frames as $s(\P_q, \P_p) >> s(\P_q, \P_n)$ and rank the candidates by the similarities of the frames in the dataset, where $s(\cdot)$ is the similarity function, and $\P_p$ and $\P_n$ are positive and negative point clouds, respectively. We want the model to treat similarities between the query frame and positive frames much higher than the similarities with negative frames.
% \vspace{-1em}
% \begin{align}
    
%     \label{eq:problem_definition}
% \end{align}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/architecture.png}
    \caption{\textbf{PoCo Architecture.} The inputs are the query and database RGBD point clouds. The Feature Extractor processes the point features and generates a global descriptor for each frame. The descriptors of the query frame are compared with descriptors of the database frames by cosine similarity, and then we rank the candidate frames according to the similarities. Note that the extractor consists of Farthest Point Sampling (FPS), an encoder, and layers Reducers and Cluster blocks (see Fig.~\ref{fig:reducer},~\ref{fig:cocs}). The FPS step processes the indices of the downsampled points in the beginning of the Feature Extractor and the following blocks sequentially apply the downsampled features.}
    \label{fig:architecture}
    \vspace{-2em}
\end{figure*}

\subsection{Architecture of Our PoCo Model}
\label{sec:architecture}

The architecture of our PoCo model is shown in Figure \ref{fig:architecture}. The inputs to our model are two types of point clouds. One is query frames $\cp_q$ and the other type contains the database frames $\cp_d$. For each point cloud $\P_i\in \cp_q$ and each $\P_j \in \cp_d$, the dimension is $N\times 9$, where the second dimension represents the point feature, which includes RGB $\set{r, g, b}$, Position $\set{x, y, z}$ and Normals $\set{n_x, n_y, n_z}$. In this approach, we extend the concept of Context Clusters~\cite{cocs} to point cloud, so our general architecture contains a sequence of Point Reducer and Context Cluster blocks.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figs/place_holder.png}
%     \caption{Reducer Block}
%     \label{fig:reducer}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/pcf_cocs.png}
    \caption{\textbf{Reducer Block.} The blue circles are points in different levels. In Reducer Block, we use Farthest Point Sampling method to downsample points and use PointConvFormer to aggregate the geometric and feature information of the K-nearest neighbors to the downsampled points. The downsampled points are also used as centers of the last layer Cluster Block to help feature processing.}
    \label{fig:reducer}
    \vspace{-1.5em}
\end{figure}

\textbf{Reducer Blocks:} Each reducer block is used to perform two functionalities: 1. aggregate the features of the points from the last layer to the current layer; 2. process the geometric and feature relationship among the points in the current layer. The aggregation computation in the reducer blocks is based on the PointConvFormer~\cite{wu2023pointconvformer}. Denote the point cloud in layer $l$ as $\P^l$. $\P^l$ contains features with shape $N\times D$, where $D$ is the dimension of feature space and $N$ is the number of points. The geometric information has the shape $N\times G$, where $G=\left |{x, y, z, n_x, n_y, n_z}\right |$, where $\n = \set{n_x, n_y, n_z}$ is the normal vector of the point. Firstly, we down-sample the points to choose a smaller number of points for the next layer. The Farthest sampling (FPS) method~\cite{eldar1997farthest} is used to as a downsampling method to choose $M$ number of points $\P^{l+1}$ in the next layer, where $M<N$. After the downsampling, we use K-nearest-neighbor(KNN) strategy~\cite{kramer2013k} to choose the K nearest neighbors in $\P^l$ for each point $p\in \P^{l+1}$ in the next layer $\P^{l+1}$ as shown in Figure \ref{fig:reducer}. 
Then we apply one single PointConvFormer layer to aggregate the features from $\P^l$ and one single layer to process the features in point cloud $\P^{l+1}$.
% \vspace{-0.5em}
\begin{align}
    \f_p &= W_l \sum_{p_k\in \cn(p)} h(g(p_k,p))\psi(f(p_k), f(p))f(p)^\top.
    \label{eq:pointconvformer}
\end{align}
As Equation \ref{eq:pointconvformer}, for each point $p \in \P^l$, it has K nearest neighbors $p_k\in\cn(p)$, $\f_p$ represents the feature vector of a point $p$ and $f(\cdot)$ represents the features of the point processed by one linear layer. The $\psi(\cdot)$ is a multi-head attention mechanism calculating the similarity scores between $f(p_k)$ and $f(p)$. $h(\cdot)$ represents the linear layers. $g(p_k, p)$ is a vector containing coordinate independent geometric information as Equation \ref{eq:geos}, where $\r_k$ is a distance vector from point $p_k$ to $p$, $\n$ and $\n_k$ are normal vectors of points $p$ and $p_k$. This vector only contains the relative geometric information between the two points~\cite{li2021devils}.
% couldn't find the publication version of this citation.
Thus, after the reducer block, the features and geometric information would be sent to the following Context Cluster blocks.

% DO I NEED TO EXPLAIN MORE ABOUT THE \PSI(*)???
\vspace{-1em}
\begin{align}
    \hat{\r}_k = \frac{\r_k}{\norm{\r_k}}; \;\; &\v = \frac{\n_k-(\n_k\cdot \hat{\r}_k)\hat{\r}_k}{\norm{\n_k-(\n_k\cdot \hat{\r}_k)\hat{\r}_k}}; \;\; \w=\frac{\hat{\r}_k\times \v}{\norm{\hat{\r}_k\times \v}};\nonumber
\end{align}
\begin{align}
    g(p_k, p) = &[\n\cdot \n_k, \frac{\r_k\cdot \n_k}{\norm{\r_k}}, \frac{\r_k\cdot \n}{\norm{\r_k}}, \n\cdot\v, \n\cdot\w, \r_k\cdot \n_k, \nonumber\\
    &\r_k\cdot(\n\times\n_k), \norm{\r_k}], 
    \label{eq:geos}
\end{align}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/cluster.png}
    \caption{\textbf{Cluster Block.} Red points are centers downsampled from the blue points. The blue points are grouped by the similarity of w.r.t. the red centers. Then the features of the blue points are aggregated to the centers by Eq.~\ref{eq:cluster} and then the center features are dispatched to the points by Eq.~\ref{eq:dispatch}.}
    \label{fig:cocs}
    \vspace{-2em}
\end{figure}
\textbf{Cluster Blocks:} Figure \ref{fig:cocs} shows that in order to build a powerful deep neural network for point feature extraction, there are two sub-blocks in one layer of Cluster block. We reuse the downsampled points in the next layer as centers to help process the point features in the current layer. As shown in Figure \ref{fig:cocs},  $\f_c$ represents the feature of the center $c \in \cp^{l+1}$, where the centers in Cluster Block are the downsampled points in the Reducer Block in the next layer. Given $\f_c$ and features $\f_p$ of the current layer of points $p\in \cp^l$, the first step is to calculate the cosine similarity between all the centers and all the points, and then we have $s_{c,p} = \sigma(\alpha \cdot cosine(\f_p, \f_c)+\beta)$, where $\sigma(\cdot)$ is the sigmoid activation function and $\alpha$ and $\beta$ are trainable parameters. The second step is to aggregate the features of all points to all centers according to the similarities as Equation \ref{eq:cluster}
\begin{align}
    \f_c = \frac{1}{\cc} \left( \f_c + \sum_{p=1}^N  \s_{c,p} \cdot \f_p \right),
    \label{eq:cluster}
\end{align}
$\cc=1+\sum_{p=1}^N \s_{c,p}$. The weighted aggregation of the local point features provides higher-level center features, and then the higher-level information can be used to enhance the local features. So in the next step, the same similarity values are used to dispatch the center features to local points, as Equation \ref{eq:dispatch}:
\vspace{-0.5em}
\begin{align}
    \f_p = \f_p + h(s_{c,p} \cdot \f_c )).
    \label{eq:dispatch}
\end{align}
In this way, we extend the concept of Context Clusters~\cite{cocs} to process the point cloud features.

\textbf{Global Descriptor Model:} The last layer of the PoCo model is to aggregate all the point features together and generate a global descriptor for the point cloud. The global descriptor is finally used to calculate the similarity between the query frame and candidate frames in a database. In our approach, we use cosine similarity to compare the global descriptors and recognise if the candidate frames match the query frame. In this model, we use a Reducer Block, but with only one point in the next layer's point cloud. The input point features of the Global Descriptor Model are all normalized and aggregated by the geometric and feature weights as Equation \ref{eq:pointconvformer}. The output global descriptor of this model is the vector $\g$ with a dimension of 256.

\subsection{Training}
\label{sec:training}
Previous place recognition tasks only rank the candidate frames without calculating the similarity score between the candidate frames and the query frame (with global descriptor $\g_q$). In comparison, PoCo recognise the difference between positively matched frames (with global descriptor $\g_p$) and negatively matched frames (with global descriptor $\g_n$) and also computes the difference scores between each query-candidate pair. This function is achieved by using both Circle Loss~\cite{sun2020circle} and Triplet Loss~\cite{schroff2015facenet}. 

In Equation \ref{eq:circle}, $softplus(\cdot)$ is the soft plus function. Function $cl(\cdot)$ represents the clamp minimum, where the value is clamped by 0. The $m=0.2$ is the margin. $\gamma=1$ is a hyperparameter. $s_p$ and $s_n$ are similarities between the query frame and the matched frames and not matched frames, respectively, and the similarity is calculated by cosine similarity between the global descriptors.

\begin{align}
    a_p = cl(-s_p+1-m, 0), a_n = cl(s_n+m, 0) \\
    \cl_c = softplus(\log \sum \exp(\gamma a_n (s_n - \delta_n)) - \\
    \log \sum \exp(\gamma a_p (s_p - \delta_p)))
    \label{eq:circle}
\end{align}

As Equation \ref{eq:triplet}, triplet loss, $\cl_t$, uses L2 distance, $d(\cdot)$, to calculate the distances between global descriptors of query frame and database frame. $m=0.2$ is the margin.

\begin{align}
    \cl_t = \max(d(\g_p, \g_q) - d(\g_n, \g_q) + m, 0)
    \label{eq:triplet}
\end{align}

In the final loss function, we combine the two losses $\cl = \alpha \cl_c + \beta \cl_t$. During training, the candidate is mostly ranked by the similarity of the candidate frames so computing the difference between matched frames and not matched frames is the most important, therefore, the triplet loss is the major loss. We give a large weight to triplet loss, $\alpha=10$, and smaller weight to circle loss, $\beta=0.1$.

\section{Experiments}

\subsection{Dataset and Implementation}
Our approach is trained and evaluated by the ScanNet-PR~\cite{ming2022cgis} database, which is derived from the ScanNet dataset~\cite{dai2017scannet}. The ScanNet-PR database is an indoor database, where each scenario is captured in one room with multiple frames. Each frame contains RGB and point cloud (xyz) information. For different frames, the number of points is different based on how rich are the features in the frame. There are 807 scenarios in total split into training (565), validation (142), and testing (100) datasets.

Our PoCo model is implemented by Pytoch and trained on the 8 Tesla-V100 GPUs. All the input point numbers of each frame are constrained to 2000 points, and if the point number is larger than the threshold, we use random select 2000 points from the point cloud. The normal vector of each point in the point cloud is calculated by all the points within the radius of 0.2 meters. In our system, we use cosine annealing scheduler~\cite{loshchilov2016sgdr} with Adam optimizer~\cite{kingma2014adam}. The increase factor of the scheduler is $1$ and learning rate starts from $10^{-4}$ to $10^{-7}$. 


% OTHER IMPORTANT PARAMETERS OF THE MODEL ARCHITECTURE after drawing figures

In our implementation, besides the complete PoCo model, we also designed a Vanilla RGB model based on the CoCs feature extractor. We use the CoC-Medium~\cite{cocs} as the backbone and in the last layer, we apply another reducer, where we apply a 2D-convolutional layer to the centers from the last layer of CoC-Medium and output a global descriptor with the dimension of 256. Another model for ablation study is the PoCo w/o color, where we only use coordinates and normals as the input feature of each point and process the features by our PoCo architecture. 

CGiS-Net is the baseline method to compare with. We are following the same experiment setup as CGis-Net work. To be specific, the recall values are calculated on the testing dataset, where the candidate point clouds are chosen by a distance threshold of 3 meters. Given a query frame, we calculate the similarities of the candidate global descriptors with the descriptor of the query frame and then rank the candidate frames according to the similarity. The standard evaluation metric Recall @ K is calculated by the percentage of correctly matched query frames given to top K candidates. Besides CGiS-Net, we also compared with NetVLAD~\cite{arandjelovic2016netvlad}, Indoor DH3D~\cite{du2020dh3d} and MinkLoc3D~\cite{komorowski2021minkloc3d}. We present the quantitative results (recall@K) on the ScanNet-PR dataset in Table \ref{tab:recall} and show qualitative comparisons from different room environments.

We evaluate the running time (inference time) of the global descriptor generation for a single frame. We use the device with one NVIDIA RTX A5000 GPU and an Intel Xeon(R) W-2255 CPU. Our PoCo model takes around 12ms, which outperforms the CGiS-Net, which takes 23ms for each step. Our PoCo method is around \textbf{2}$\times$ faster than CGiS-Net.

\input{qualitative}

\subsection{Recall Values}
We evaluate the performance of our method by comparing with baseline methods, CGiS-Net~\cite{ming2022cgis}, MinkLoc3D~\cite{komorowski2021minkloc3d}, DH3D~\cite{du2020dh3d}, PointNetVLAD~\cite{uy2018pointnetvlad}, NetVLAD~\cite{arandjelovic2016netvlad} and SIFT feature with Bag of Words~\cite{sivic2008efficient}. As shown in Table \ref{tab:recall}, our full PoCo model outperforms the other approaches by at least $5.7\%$. We also evaluate the effect of different types of features on the final results, so we apply the ablation studies by using only RGB color features and only geometric features. Our PoCo model w/o color achieves around $5\%$ improvement compared with CGiS-Net w/o color and the PoCo model w/o geometry outperforms CGiS-Net w/o geometry by around $2\%$. The results means not only can our model effectively embed the geometric information of the point cloud, but also process color features better than the other state-of-the-art method. From the table, we can also notice that the PoCo w/o color is better than PoCo w/o geometric, which means geometric information plays an important role in the place recognition task.

\begin{table}[h!]
    \centering
    \begin{tabular}{c|c|c|c}
ScanNetPR & R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$\\
\hline
\hline
SIFT~\cite{david2004distinctive} + BoW~\cite{sivic2008efficient} & 16.16 & 21.17 & 24.38 \\
\hline
NetVLAD~\cite{arandjelovic2016netvlad} & 21.77 & 33.81 & 41.49 \\
\hline
PointNetVLAD~\cite{uy2018pointnetvlad} & 5.31 & 7.50 & 9.99 \\
\hline
Indoor DH3D~\cite{du2020dh3d} & 16.10 & 21.92 & 25.30 \\
\hline
MinkLoc3D~\cite{komorowski2021minkloc3d} & 3.32 & 5.81 & 8.27 \\
\hline
\hline
CGiS-Net~\cite{ming2022cgis} & 61.12 & 70.23 & 75.06 \\
\hline
CGiS-Net w/o color~\cite{ming2022cgis} & 39.62 & 50.92 & 56.14 \\
\hline
CGiS-Net w/o geometry~\cite{ming2022cgis} & 40.07 & 51.28 & 58.96 \\
\hline
\hline
Vanilla RGB CoCs~\cite{cocs} & 41.82 & 57.65 & 66.82 \\
\hline
PoCo w/o color & 44.34 & 54.27 & 59.78 \\
\hline
PoCo w/o Equation~\ref{eq:geos} & * & * & * \\
\hline
PoCo & \textbf{64.63} & \textbf{75.02} & \textbf{80.09} \\
    \end{tabular}
    \caption{The table shows our PoCo method outperforms baseline models w.r.t recall @ K. For R@1, our Vanilla RGB outperforms the CGiS-Net w/o geometry around $2\%$ and our PoCo w/o color outperforms CGiS-Net w/o color around $5\%$. It is worth to highlight that being different from CGis-Net, PoCo doesn't use any semantic segmentation ground truth labels in our training stage.} 
    \label{tab:recall}
    \vspace{-1em}
\end{table}

\begin{table}[h!]
    \centering
    \begin{tabular}{c|c|c|c}
ARKit & R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$\\
\hline
\hline
PointNetVLAD~\cite{uy2018pointnetvlad} & * & * & * \\
\hline
MinkLoc3D~\cite{komorowski2021minkloc3d} & * & * & * \\
\hline
CGiS-Net~\cite{ming2022cgis} & * & * & * \\
\hline
\hline
Vanilla RGB CoCs~\cite{cocs} & * & * & * \\
\hline
PoCo w/o color & * & * & * \\
\hline
PoCo w/o Equation~\ref{eq:geos} & * & * & * \\
\hline
PoCo & * & * & * \\
    \end{tabular}
    \caption{} 
    \label{tab:recall}
    \vspace{-1em}
\end{table}


\subsection{Qualitative Results}
In this section, we show the comparisons between our approach and the CGiS-Net in qualitative pictures and we also evaluate how geometric and color information affect the performance. 

As shown in Figure \ref{fig:qualitative_results}, our PoCo model can find the best-matched frames even though the overlap area is very small, as the red circles marked in the figure. Figure \ref{fig:geometric_results} shows how geometric information helps in the place recognition task. As shown in Figure \ref{fig:geometric_results}, the Vanilla-RGB-PR model can detect objects, such as chairs and washing machines, but it cannot recognize the relative positions of the objects very well. The complete PoCo model can effectively handle the geometric relations of the objects in the scenarios. Figure \ref{fig:color_results} shows the comparison between the complete PoCo and PoCo w/o Color, where only geometric information is used in the model. As shown in the figure, we can see the PoCo w/o Color is capable of recognizing very similar structures, such as the table and the chair in the first row, and the bed in the second row. But because it doesn't have color information, it falsely matched the frames with very obvious color differences. The complete PoCo model can effectively combine the color and geometric information in the recognition task.


% \subsection{Computational Evaluation}

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|c|c}
% & FLOPs & Latency \\
% \hline    
% CGiS-Net & & \\
% \hline
% PoCo    & &
%     \end{tabular}
%     \caption{Computational Results}
%     \label{tab:compuatational_results}
% \end{table}



\section{Conclusion, Limitations and Future Work}
We are the first to propose a Point-Cloud-based place recognition model based on the concept of CoCs. We explicitly encode geometric information during feature extraction with transformer-based models. PoCo outperforms previous indoor RGBD place recognition methods significantly in recall@K. However, our model still has its limitations, where sometimes our model relies much on the geometric information that hurts the performance and in some extreme cases where the overlapping areas between the ground truth and query frame are small and do not have many features. To solve the issues, we could use local features to help reranking candidate frames to improve accuracy. Therefore, in the future, a second stage of re-ranking candidates will be explored.

% \section*{ACKNOWLEDGMENT}

